On the Performance of Multidimensional Constellation Shaping for Linear and Nonlinear Optical Fiber Channel

Multidimensional constellation shaping of up to 32 dimensions with different spectral efficiencies are compared through AWGN and fiber-optic simulations. The results show that no constellation is universal and the balance of required and effective SNRs should be jointly considered for the specific optical transmission scenario.

==> tex/Table.tex <==
\def\arraystretch{0.9}
\begin{table}[!tb]
\centering
\caption {Simulation parameters.}
\vspace{-1em}
\begin{center}
\label{tab:para}
% \scalebox{0.9}{
{\footnotesize
\begin{tabular}{c|c}
\hline
% \toprule
% \multicolumn{1}{c}{\bf Parameter name} & {\bf Value}  \\
{\bf Parameter name} & {\bf Value}\\
\hline
% \hline
\multicolumn{2}{c}{\bf TX parameters}\\
\hline
No. of channels & 1    \\
\hline
Symbol rate & {45~GBd}   \\
\hline
RRC roll-off  & {0.01}{\%} \\
\hline
\multicolumn{2}{c}{\bf Fiber parameters}\\
\hline
Attenuation & {0.2~(dB/km)} \\
\hline
Dispersion parameter & {-21.683~(ps$^2$/km)} \\
\hline
Nonlinearity parameter & {1.3~(w.km)$^{-1}$} \\
\hline
EDFA noise figure & {5~dB} \\
\hline
\multicolumn{2}{c}{\bf Link parameters}\\
\hline
Fibre span length & {80~km} \\
\hline
No. of spans & {100}\\
\hline
\multicolumn{2}{c}{\bf SSFM parameters}\\
\hline
Step size & {0.1~km}\\
\hline
Samples per symbol &{4}\\
\hline
% \toprule
\end{tabular}
}
% }
\end{center}
\end{table}
